HashMem: PIM-based Hashmap Accelerator

Hashmaps are widely utilized data structures in many applications to perform a probe on key-value pairs. However, their performance tends to degrade with the increase in the dataset size, which leads to expensive off-chip memory accesses to perform bucket traversals associated with hash collision. In this work, we propose HashMem, a processing-in-memory (PIM) architecture designed to perform bucket traversals along the row buffers at the subarray level. Due to the inherent parallelism achieved with many concurrent subarray accesses and the massive bandwidth available within DRAM, the execution time related to bucket traversals is significantly reduced. We have evaluated two versions of HashMem, performance-optimized and area-optimized, which have a speedup of 49.1x/17.1x and 9.2x/3.2x over standard C++ map and hyper-optimized hopscotch map implementations, respectively.

==> Sections/MotivationAndKeyIdea.tex <==
\section{Motivation and Key Idea}

The probing operations to a HashMap tends to generate random addresses along with low data reuse (i.e. hash-bucket data being scanned and discarded if not required). Due to the randomness of the memory addresses being probed, the prefetching mechanism cannot accurately predict the data to be accessed in advance leading to pipeline stalls and degraded performance. The hash buckets in turn stream a large chunk of data from the off-chip DRAM to perform a simple array scan operation that results in lot of data being discarded after a single comparison operation while at the same time traversing all the way through the cache hierarchy. 
Clearly, we observe that if there exists a mechanism to implement the efficient probing operation of a hashmap and extract data of interest related to a specific key without the overheads detailed above, this would translate into improved performance for applications performing frequent hashmap probes. 

We observe that process-in-memory architectures place compute elements either in-situ or near the data to perform processing operations to where the data resides. This not only enables making use of massive parallelism and immense bandwidth available within the DRAM hierarchy, but it also avoids expensive DRAM transfers across the memory bus. However, integrating complex logic on the same substrate as memory has considerable challenges, both manufacturing and thermal constraints. Hence, PIM architectures with simpler logic such as ALU or smaller fixed function blocks are proposed to be placed within the memory to enable PIM functionality. 

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/memorymap.png}
  \caption{Mapping Key-Value pairs to PIM-enabled memory subarrays}
  \Description{Mapping Key-Value pairs to PIM-enabled memory subarrays}
  \label{fig:subarray_translation}
\end{figure}

We observe that hashmap traversals involve selecting a bucket and comparing the hash nodes individually until a key of interest is reached. These comparison operations are extremely suitable for the small ALU units residing within the PIM structures while at the same time, the bandwidth available within the DRAM could be leveraged for faster access and probing of hashnodes. We furthermore observe that the subarray layout within the DRAM is the physical realization of a hashmap data structure construct where the rows translate into a hash bucket while columns translate into the hash nodes. We aim to leverage these similarities within the DRAM hierarchy to implement an efficient PIM architecture to accelerate the probing operations on a hashmap as illustrated in Figure-\ref{fig:subarray_translation}.


